Dual Diffusion for Unified Image Generation and Understanding

Diffusion models have gained tremendous success in text-to-image generation, yet still lag behind with visual understanding tasks, an area dominated by autoregressive vision-language models. We propose a large-scale and fully end-to-end diffusion model for multi-modal understanding and generation that significantly improves on existing diffusion-based multimodal models, and is the first of its kind to support the full suite of vision-language modeling capabilities. Inspired by the multimodal diffusion transformer (MM-DiT) and recent advances in discrete diffusion language modeling, we leverage a cross-modal maximum likelihood estimation framework that simultaneously trains the conditional likelihoods of both images and text jointly under a single loss function, which is back-propagated through both branches of the diffusion transformer. The resulting model is highly flexible and capable of a wide range of tasks including image generation, captioning, and visual question answering. Our model attained competitive performance compared to recent unified image understanding and generation models, demonstrating the potential of multimodal diffusion modeling as a promising alternative to autoregressive next-token prediction models.

==> sec/X_suppl_separate.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

% \section{Rationale}
% \label{sec:rationale}
% % 
% Having the supplementary compiled together with the main paper means that:
% % 
% \begin{itemize}
% \item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
% \item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
% \item When submitted to arXiv, the supplementary will already included at the end of the paper.
% \end{itemize}
% % 
% To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.

\section{Training Details}
\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{ccccc} 
\toprule
\multirow{2}{*}{Hyperparam.} & \multirow{2}{*}{Dual pretrain} & \multicolumn{2}{c}{Continued pretrain} & \multirow{2}{*}{Instruct. tuning} \\ 
\cmidrule{3-4}
 &  & Mask emb. & High res. &  \\ 
\midrule
Gradient steps & 60k & 200k & 80k & 50k \\
Batch size & 512 & 512 & 768 & 512 \\
LR & 5e-5 & 3e-5 & 3e-5 & 3e-5 \\
Scheduler & \multicolumn{4}{c}{Constant LR with warmup} \\
Warmup iters & 5000 & 1000 & 1000 & 1000 \\
Weight decay & \multicolumn{4}{c}{1e-2} \\
Text loss weight & \multicolumn{3}{c}{0.2} & 1.0 \\
\bottomrule
\end{tabular}}
\caption{Training hyperparameters for D-DiT. Text loss weight denotes the $\lambda$ in Equation (8).}
\label{tab:training hyperparam}
\end{table}

We provide the detailed hyperparameter setting for different training stages in the Table \ref{tab:training hyperparam}. During all the training stages, we use AdamW optimizer with default hyperparameters ($\beta_1=0.9, \beta_2=0.999$). Mixed precision training (bf16) and fully-sharded data parallel (with gradient and optimizer state sharded) are used for model training.

\section{Further Results}
\begin{table}[h]
\centering
\begin{tabular}{cccc} 
\toprule
Model & Backbone & Params. (B) & FID $\downarrow$ \\ 
\midrule
SD-XL \citep{podell2023sdxl} & Diff. & 0.9 & 9.55 \\
PixArt-$\alpha$ \citep{chen2023pixart} & Diff. & 0.6 & 6.14 \\
Playground v2.5 & Diff. & - & 4.48 \\
Show-O \citep{xie2024show} & Discrete Diff. & 1.3 & 15.18 \\
LWM \citep{liu2024lwm} & AR & 7 & 17.77 \\
VILA-U \citep{wu2024vila} & AR & 7 & 7.69 \\ 
\midrule
SD3 \citep{esser2024scaling} & Diff. & 2 & 16.45 \\
D-DiT & Diff. & 2 & 15.16 \\
\bottomrule
\end{tabular}
\caption{Comparison with other models
on MJHQ-30K evaluation benchmark at $512\times512$ resolution.}
\label{tab:mjhq fid}
\end{table}

\begin{table}[h]
\centering
\fontsize{9.5pt}{9.5pt}\selectfont
\begin{tabular}{cccccc} 
\toprule
\setlength{\tabcolsep}{2.0pt}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{COCO-30k} & \multicolumn{3}{c}{T2I CompBench} \\ 
\cmidrule(lr){2-3}\cmidrule(lr){4-6}
 & FID $\downarrow$ & CLIP $\uparrow$ & Color $\uparrow$ & Shape $\uparrow$ & Texture $\uparrow$ \\ 
\midrule
SD3 & 10.2 & 30.9 & 0.7993 & 0.5816 & 0.7389 \\
D-DiT & 9.4 & 31.2 & 0.8001 & 0.5703  & 0.6856 \\
\bottomrule
\end{tabular}
\caption{Further image generation comparisons against original SD3 on MS-COCO dataset \citep{lin2014mscoco} and T2I CompBench \citep{huang2023t2i}.}
\label{table:sd3_comparison}
\end{table}

\paragraph{Image generation} We evaluate the aesthetic quality of generated images from our proposed D-DiT against those of the original SD3 model and a selection of existing text-to-image (T2I) and multi-modal works. We measure Frechet Inception Distance (FID) with respect to a collection highly aesthetic generated images, known as the MJHQ-30K benchmark proposed by \citep{li2024playground}. As shown in Table \ref{tab:mjhq fid}, we observe an improvement in FID after joint diffusion training, and favorable comparison against multi-modal models of similar size. We also provide further comparisons on MS-COCO 30k and T2I CompBench in Table \ref{table:sd3_comparison}. The FID and CLIP score slightly improve compared to the original SD3 model. On T2I CompBench, we find that after dual diffusion fine tuning the model performs worse in texture. We hypothesize that the major reason is the texture quality of our training dataset is worse than the dataset used for training SD3.

\paragraph{Text generation process} We provide an illustrative example of masked diffusion in Figure \ref{fig:supp_text_flow} for the visual question answering task, where the token generation process is visualized over diffusion time. Over the course of sampling, the answer tokens are gradually denoised from the masked state via absorbing state reverse diffusion. The question tokens are always left unmasked throughout the entire process.

\begin{table}[h]
\centering
\fontsize{9pt}{9pt}\selectfont
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{ccccccc} 
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# \\trainable\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Text \\encoder\end{tabular}} & \multirow{2}{*}{Geneval} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}COCO \\FID\end{tabular}} & \multicolumn{2}{c}{VQAv2(val)} \\ 
\cmidrule(lr){6-7}
 &  &  &  &  & 0-shot & 32-shot \\ 
\midrule
End-to-End & 1.1B & - & 0.39 & 18.1 & 54.3 & 58.7 \\
From SD3 & 2B & T5-XXL & 0.65 & 9.4 & 55.0 & 60.3 \\
\bottomrule
\end{tabular}
\caption{Comparison of different D-DiT variants.  \textit{End-to-End} variant is trained from scratch and uses GPT2's text tokenizer. \textit{From SD3} variant is  initialized from SD3 pretrained checkpoint and uses T5 encoder. The end-to-end model is first trained on OpenWebText for 350B tokens, then trained on DataComp-recap1B for an epoch (400k steps) and a filtered subset for 100k steps. \label{tab:end2end_ablation}}
\end{table}

\paragraph{Training from scratch and removing T5 encoder} To study the influence of text-to-image pretraining, we conduct a study by comparing a D-DiT model that is trained from scratch. We found that initializing from pretrained text-to-image model and use a pretrained text encoder can greatly aid model learning of text-to-image tasks. Meanwhile, image captioning on VQA also mildly improves (Table \ref{tab:end2end_ablation}).


\paragraph{Image generation's influence on SFT} To analyze the influence of dual diffusion loss on image understanding, we conduct supervised finetune on LLaVA 1.5 dataset with varying amount of image generation data, including a training that only has understanding loss (no generation data). We observe that the image generation loss and corresponding data amount
does not have significant influence on model's understanding performance (Table \ref{table:data_ablation}).

\begin{table}[h]
\centering
\fontsize{9.0pt}{9.0pt}\selectfont
\begin{tabular}{cccccccc} 
\toprule
\multirow{2}{*}{Und.} & \multirow{2}{*}{Gen.} & \multicolumn{3}{c}{VQAv2 (val)} & \multicolumn{3}{c}{POPE} \\ 
\cmidrule(r){3-5}\cmidrule(r){6-8}
 &  & 10k & 30k & 50k & 10k & 30k & 50k \\ 
\midrule
0.665M & 0 & 52.8 & 55.9 & 58.3 & 79.6 & 80.9 & 81.8 \\
0.665M & 7M & 53.4 & 55.8 & 58.1 & 79.8 & 81.2 & 82.4 \\
0.665M & 20M & 53.6 & 55.8 & 58.3 & 81.0  & 81.1 & 82.5 \\
\bottomrule
\end{tabular}
\vspace{-.14in}
\caption{Understanding performance (accuracy) under different data settings and training steps during supervised finetune. Batch size is set to 128 for this experiment.}
\label{table:data_ablation}
\end{table}

\paragraph{Comaprison against previous multi-modal diffusion model} We also include a qualitative comparison in captioning performance compared to UniDiffuser \citep{bao2023unidiffuser}, another diffusion-based multi-modal model, in Figure \ref{fig:supp_i2t}, where we demonstrate an improvement in the ability to capture fine-grained details of the image in a longer caption format. Finally, we provide further uncurated text-to-image (T2I) generation results in Figures \ref{fig:supp_t2i}, \ref{fig:supp_t2i_2}, \ref{fig:supp_t2i_3}, and \ref{fig:supp_t2i_4}. Overall, these results further demonstrate the multi-faceted performance of our proposed dual-branch diffusion-based multi-modal model.

\begin{figure*}[t]
\centering
    \begin{subfigure}[B]{0.49\linewidth}
        \centering
\includegraphics[width=0.80\linewidth]{figures/annotated_t2i_failure.png}
    \caption{ T2I Prompt: \textit{Three trucks parking in parallel: one red, one blue, and one white. Red truck has load and the rest don't have. }   \label{fig:t2i failure}}
    \end{subfigure}
    \begin{subfigure}[B]{0.5\linewidth}
        \centering
    \includegraphics[width=\linewidth]{figures/annotated_i2t_failure.png}
    \vspace{+0.5mm}
    \caption{ I2T Prompt:\textit{Q: How many pens are there on the desk and what are their colors?} A: There are three pens on the desk, and they are red and blue.    \label{fig:i2t failure}}
    \end{subfigure}
    \caption{Examples of failed text-to-image and image-to-text generation.}
\end{figure*}

\paragraph{Limitations} 

As shown in Figure~\ref{fig:i2t failure}:
in T2I, we find that D-DiT can struggle to generate scenes with relatively complex instructions. In I2T, D-DiT can fail to identify the full details of smaller objects. We also observe model's performance performance deteriorates with longer prompts, primarily due to the bias towards short prompts in the LLaVA finetuning dataset.

In summary, while discrete diffusion offers the advantage of being agnostic to sequential order and is compatible with bi-directional Transformers, its current implementation requires the sequence length to be preset before sampling. A promising future direction would be to extend the sampling scheme to allow for more flexibility, enabling dynamic sequence lengths during the sampling process. 
In addition, while we show that our proposed dual diffusion model can perform instruction tuning, its instruction-following capabilities still marginally lag behind those of state-of-the-art autoregressive models.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/vqa_flow_example.pdf}
    \vspace{-1mm}
    \caption{Illustrative example of visual question answering with mask diffusion.}
    \label{fig:supp_text_flow}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.97\linewidth]{figures/caption_example.pdf}
    \vspace{-1mm}
    \caption{Comparison of captions generated by D-DiT and UniDiffuser\citep{bao2023unidiffuser}. The prompt to D-DiT is "Provide a brief description of the given image."}
    \label{fig:supp_i2t}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ex1.jpg}
        \vspace{-7mm}
    \caption{Additional text-to-image samples generated from the model.}
    \label{fig:supp_t2i}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ex2.jpg}
        \vspace{-7mm}
    \caption{Additional text-to-image samples generated from the model.}
    \label{fig:supp_t2i_2}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ex3.jpg}
        \vspace{-7mm}
    \caption{Additional text-to-image samples generated from the model.}
    \label{fig:supp_t2i_3}
    \vspace{-3mm}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ex4.jpg}
        \vspace{-7mm}
    \caption{Additional text-to-image samples generated from the model.}
    \label{fig:supp_t2i_4}
    \vspace{-3mm}
\end{figure*}

